On the Rankin-Selberg $L$-factors for ${\rm SO}_{5}\times{\rm GL}_2$

Let $\pi$ and $\tau$ be a smooth generic representation of ${\rm SO}_5$ and ${\rm GL}_2$ respectively over a non-archimedean local field. Assume that $\pi$ is irreducible and $\tau$ is irreducible or induced of Langlands' type. We show that the $L$- and $\epsilon$-factors attached to $\pi\times\tau$ defined by the Rankin-Selberg integrals and the associated Weil-Deligne representation coincide. Similar compatibility results are also obtained for the local factors defined by the Novodvorsky's local zeta integrals attached to generic representations of ${\rm GSp}_4\times{\rm GL}_2$.

==> SO(5)xGL(2)/amssymbol.tex <==
\usepackage{amsmath}
\usepackage{amscd,amsthm,amssymb,amsfonts}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{stmaryrd}
\usepackage{euscript}
\usepackage{expdlist}
\usepackage{enumerate}

%\usepackage{enumitem}
%\usepackage[mathscr]{eucal}
% either use \mathscr (no euscript package), or use \EuScript (no eucal
% package), they are the same font
\input xy
%\xyoption{all}
%\setlength{\topmargin}{-0.4in}
%\setlength{\headheight}{8pt} \setlength{\textheight}{9in}
%\setlength{\oddsidemargin}{-0.15in}
%\setlength{\evensidemargin}{-0.15in} \setlength{\textwidth}{6.6in}
%\usepackage[OT2,T1]{fontenc}

% newcommands for thesis
%\renewcommand{\thesubsubsection}{\thesubsubsection}
%\newcommand{\mysubsection}[1]{\subsection[#1]{\normalfont\itshape #1}}
%\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-3.25ex plus -1ex minus -.2ex}{1.5ex plus .2ex}{\normalsize\itshape}}
%\newcommand{\mysubsubsection}{\subsubsection}
% theorems, lemmas,..
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\renewcommand{thethm}{\arabic{section}.\arabic{subsection}}
\newtheorem{thmA}{Theorem}
\renewcommand{\thethmA}{\Alph{thmA}}
\newtheorem{corA}{Corollary}
\renewcommand{\thecorA}{\Alph{thmA}}
\newtheorem{hypA}{Hypothesis}
\renewcommand{\thehypA}{\Alph{hypA}}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem*{thma}{Theorem A}
\newtheorem*{thmb}{Theorem B}
\newtheorem*{thmc}{Theorem C}
\newtheorem*{thmd}{Theorem D}
\newtheorem*{thm*}{Theorem}
\newtheorem*{say}{Say}
\newtheorem{lm}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{cor*}{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem*{conj*}{Conjecture}
\newtheorem{conj}{Conjecture}

%proposal
\newtheorem{expected_thm}{Expected theorem}
\newtheorem{consequence}{Consequence}

\newtheorem{I_thm}{Theorem} % Used in Introduction
\newtheorem{I_cor}{Corollary} % Used in Introduction

\theoremstyle{remark}
\newtheorem*{remarks}{Remarks}
\newtheorem*{remark}{Remark}
\newtheorem{I_remark}{Remark} % Used in Introduction
\newtheorem*{thank}{Acknowledgments}
\newtheorem*{Notation}{Notation}

\theoremstyle{definition}
\newtheorem{I_defn}{Definition} % Used in Introduction
\newtheorem*{defn*}{Definition}
\newtheorem{Remark}[thm]{Remark}
\newtheorem{I_Remark*}{Remark}
\newtheorem{defn}[thm]{Definition}
\newtheorem{EX}{Exercise}
\newtheorem{example}[thm]{Example}
\newtheorem{problem}{Problem}

\newtheorem{hypothesis}[thm]{Hypothesis}
\newtheorem*{hypR}{Hypothesis R}
\renewcommand{\thehypothesis}{\Alph{hypothesis}}


%for temporary use
\newcommand{\nc}{\newcommand}
\newcommand{\renc}{\renewcommand}

%Convenient command
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bpmx}{\begin{pmatrix}}
\newcommand{\epmx}{\end{pmatrix}}
\newcommand{\bbmx}{\begin{bmatrix}}
\newcommand{\ebmx}{\end{bmatrix}}
\newcommand{\wh}{\widehat}
\newcommand{\wtd}{\widetilde}
\newcommand{\thetalift}[2]{\theta_{#1}(#2)}
%\newcommand{\bsp}{\begin{split}}



%\newcommand{\esp}{\end{split}}
%\newcommand{\beqcd}[1]{\begin{equation*}\label{#1}\tag{#1}}
%\newcommand{\eeqcd}{\end{equation*}}
%\renewcommand{\theequation}{\thesection\thesubsection\thesubsubsection.\arabic{equation}}
%\numberwithin{equation}{section}
%\newenvironment{mylist}{
%  \begin{enumerate}{}{%
%      \setlength{\itemsep}{5pt} \setlength{\parsep}{0in}
 %     \setlength{\parskip}{0in} \setlength{\topsep}{0in}
 %     \setlength{\partopsep}{0in}
  %    \setlength{\leftmargin}{0.17in}}}{\end{enumerate}}

%\newenvironment{myP}{
%  \begin{description}[\breaklabel\setlabelstyle{\bfseries}]}{\end{description}}


% references
\def\parref#1{\ref{#1}}
\def\thmref#1{Theorem~\parref{#1}}
\def\expectthmref#1{Expected theorem~\parref{#1}}
\def\propref#1{Proposition~\parref{#1}}
\def\corref#1{Corollary~\parref{#1}}     \def\remref#1{Remark~\parref{#1}}
\def\secref#1{\S\parref{#1}}
\def\chref#1{Chapter~\parref{#1}}
\def\lmref#1{Lemma~\parref{#1}}
\def\subsecref#1{\S\parref{#1}}
\def\defref#1{Definition~\parref{#1}}
\def\assref#1{Assumption~\parref{#1}}
\def\hypref#1{Hypothesis~\parref{#1}}
\def\subsubsecref#1{\S\parref{#1}}
\def\egref#1{Example~\parref{#1}}
\def\exref#1{Exercise~\parref{#1}}
\def\conjref#1{Conjecture~\parref{#1}}
\def\makeop#1{\expandafter\def\csname#1\endcsname
  {\mathop{\rm #1}\nolimits}\ignorespaces}
%\def\thmref#1{Theorem\hyperref[#1]{\ref{#1}}}

%\newenvironment{list2}{
 % \begin{list}{$\bullet$}{%
 %     \setlength{\itemsep}{0in}
 %     \setlength{\parsep}{0in} \setlength{\parskip}{0in}
 %    \setlength{\topsep}{0in} \setlength{\partopsep}{0in}
 %    \setlength{\leftmargin}{0.2in}}}{\end{list}}




%Reserved Key words
\makeop{Hom}   \makeop{End}   \makeop{Aut}   %\makeop{Isom}
\makeop{Pic} \makeop{Gal}       \makeop{Div} \makeop{Lie}
\makeop{PGL}   \makeop{Corr} \makeop{PSL} \makeop{sgn} \makeop{Spf}
 \makeop{Tr} \makeop{Nr} \makeop{Fr} \makeop{disc}
\makeop{Proj} \makeop{supp} \makeop{ker}   \makeop{Im} \makeop{dom}
\makeop{coker} \makeop{Stab} \makeop{SO} \makeop{SL} \makeop{SL}
\makeop{Cl}    \makeop{cond} \makeop{Br} \makeop{inv} \makeop{rank}
\makeop{id}    \makeop{Fil} \makeop{Frac}  \makeop{GL} \makeop{SU}
\makeop{Trd}   \makeop{Sp} \makeop{Tr}    \makeop{Trd} \makeop{Res}
\makeop{ind} \makeop{depth} \makeop{Tr} \makeop{st} \makeop{Ad}
\makeop{Int} \makeop{tr}    \makeop{Sym} \makeop{can} \makeop{SO}
\makeop{torsion} \makeop{GSp} \makeop{Tor}\makeop{Ker} \makeop{rec}
\makeop{Ind} \makeop{Coker}
 \makeop{vol} \makeop{Ext} \makeop{gr} \makeop{ad}
 \makeop{Gr}\makeop{corank} \makeop{Ann}
\makeop{Hol} %Holomorphic
\makeop{Fitt} \makeop{Mp} \makeop{CAP}
\def\Jac{\mathrm{Jac}}
%\makeop{Sel}
\def\Sel{Sel}
\def\ord{{ord}}
\def\Isom{\ul{\mathrm{Isom}}}
\def\Inj{\ul{\mathrm{Inj}}}
\def\Ord{{\mathrm{ord}}}
%\def\Ord{{\operatorname{ord}}}
\def\Cov{\mathrm{Cov}}
\def\Imb{\mathrm{I}}
\def\cusp{{\mathrm{cusp}}}

%GU(3,3)
\DeclareMathOperator{\GO}{GO}
\DeclareMathOperator{\GSO}{GSO}
\def\Gsp{{\rm Gsp}}
\def\PGsp{{\rm PGsp}}
\def\MSL{\widetilde{\SL}}
%\def\GO{{\rm GO}}
%\def\GSO{{\rm GSO}}

%\DeclareMathOperator{\Spec}{Spec}
%\def\Spec{\mathrm{Spec}\,}
%\DeclareMathOperator{\Eis}{Eis}
%\DeclareMathOperator{\codim}{codim}
%\DeclareMathOperator{\length}{length}
%\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
%\DeclareSymbolFont{cyrletters}{OT2}{wncyr}{m}{n}
%\DeclareMathSymbol{\SHA}{\mathalpha}{cyrletters}{"58}



\def\makebb#1{\expandafter\def
  \csname bb#1\endcsname{{\mathbb{#1}}}\ignorespaces}
\def\makebf#1{\expandafter\def\csname bf#1\endcsname{{\bf
      #1}}\ignorespaces}
\def\makegr#1{\expandafter\def
  \csname gr#1\endcsname{{\mathfrak{#1}}}\ignorespaces}
\def\makescr#1{\expandafter\def
  \csname scr#1\endcsname{{\EuScript{#1}}}\ignorespaces}
\def\makecal#1{\expandafter\def\csname cal#1\endcsname{{\mathcal
      #1}}\ignorespaces}
% \cal is used in article, \mathcal is used in amsart

\def\doLetters#1{#1A #1B #1C #1D #1E #1F #1G #1H #1I #1J #1K #1L #1M
                 #1N #1O #1P #1Q #1R #1S #1T #1U #1V #1W #1X #1Y #1Z}
\def\doletters#1{#1a #1b #1c #1d #1e #1f #1g #1h #1i #1j #1k #1l #1m
                 #1n #1o #1p #1q #1r #1s #1t #1u #1v #1w #1x #1y #1z}
\doLetters\makebb   \doLetters\makecal  \doLetters\makebf
\doLetters\makescr
\doletters\makebf   \doLetters\makegr   \doletters\makegr
\def\pfname{\medbreak\noindent{\scshape Proof.}\enspace}%
\renewcommand{\proofname}{\pfname}
%\def\pf{\proof}
%\def\qed{\qedmark\medbreak}%
%\def\qedmark{{\enspace\vrule height 6pt width 5pt depth 1.5pt}}%

\def\semidirect{\rtimes}    \def\setminus{\smallsetminus}
\def\Gm{{\bbG}_{m}}   \def\Ga{{{\bbG}_{\rm a}}}

\def\formalgm{\widehat{\bbG}_m}
\renewcommand{\baselinestretch}{1.02}\normalsize

\def\der{{\rm der}}
\makeop{Ram} \makeop{Rep} \makeop{mass}

\def\model#1{\underline{#1}}
\def\bfproj{\mathop{\bf Proj}\nolimits}
\def\sep{{\rm sep}}
\makeop{Bl}
\def\abs#1{\left|#1\right|}
\def\norm#1{\lVert#1\rVert}
%\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
%\newcommand{\abs}[1]{\left\vert#1\right\vert}

\def\Fpbar{\bar{\mathbb F}_p}
\def\Fp{{\mathbb F}_p}
\def\Fq{{\mathbb F}_q}
\def\Qlbar{\overline{{\Q}_{\ell}}}
\def\Ql{{\Q}_{\ell}}
\def\Qpbar{\ol{\Q_p}}
\def\Qbarp{\C_p}
\def\Qp{\Q_p}
\def\Qbar{\ol{\Q}}
\def\Zbar{\ol{\Z}}
%\def\Zpbar{\ol{\Z_p}}
\def\Zbarp{\Zbar_p}
\def\Zbarlp{\Zbar_{(p)}}

\def\Zp{\Z_p}
\def\mZbar{\frakm_{\Zbar}}
\def\mZbarp{\frakm_p}
\def\diag#1{\mathrm{diag}(#1)}
\def\el{\ell}
%*************FONTS*****************

\def\Ibar{\overline{I}}
\def\Mbar{\ol{M}}
\def\Sbar{\ol{S}}
\def\Dbar{\ol{D}}
\def\fbar{\bar{f}}
\def\lbar{\bar{l}}
\def\ybar{\bar{y}}
\def\kbar{\bar{k}}
\def\rhobar{\bar{\rho}}
%basic notation

\def\rmT{{\mathrm T}}
\def\rmN{{\mathrm N}}
\def\rmF{{\mathrm F}}
\def\rmC{{\mathrm C}}
\def\rmp{{\mathrm p}}
% mathcal
\def\cA{{\mathcal A}}  %automorphic forms
\def\cB{\EuScript B}
\def\cD{\mathcal D}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}  %Hida family
\def\cG{{\mathcal G}}
\def\cL{{\mathcal L}}
\def\cH{{\mathcal H}}
\def\cI{\mathcal I}
\def\cJ{\mathcal J}
\def\cK{{\mathcal K}}  %imaginary quadratic field
\def\cM{\mathcal M}
\def\cR{{\mathcal R}}
\def\cO{\mathcal O}
\def\cS{{\mathcal S}}
\def\cf{{\mathcal f}}
\def\cW{{\mathcal W}}
\def\ca{{\mathcal a}}
\def\cZ{\mathcal Z}
\def\cX{\mathcal X}
\def\cV{{\mathcal V}}
\def\cP{{\mathcal P}}
\def\cC{\mathcal C}
\def\cJ{\mathcal J}
\def\cN{\mathcal N}
\def\cT{\mathcal T}
\def\cY{\mathcal Y}
\def\cQ{\mathcal Q}
\def\cU{\mathcal U}

\def\calX{\mathcal X}
% EuScript
\def\EucA{{\EuScript A}}
\def\EucB{\EuScript B}
\def\EucD{\EuScript D}
\def\EucE{{\EuScript E}}
\def\EucF{{\EuScript F}}  %Hida family
\def\EucG{{\EuScript G}}
\def\EucL{{\EuScript L}}
\def\EucH{{\EuScript H}}
\def\EucI{\EuScript I}
\def\EucJ{\EuScript J}
\def\EucK{{\EuScript K}}
\def\EucM{{\EuScript M}}
\def\EucR{{\EuScript R}}
\def\EucO{{\EuScript O}}
\def\EucS{{\EuScript S}}
\def\Eucf{{\EuScript f}}
\def\EucW{{\EuScript W}}
\def\EucZ{\EuScript Z}
\def\EucX{\EuScript X}
\def\EucV{{\EuScript V}}
\def\EucP{{\EuScript P}}
\def\EucC{\EuScript C}
\def\EucJ{\EuScript J}
\def\EucN{\EuScript N}
\def\EucT{\EuScript T}
\def\EucY{\EuScript Y}
\def\EucQ{\EuScript Q}
\def\EucU{\EuScript U}



%\mathbf for U(n,n)
\def\bfc{\mathbf c}

\def\bfH{\mathbf H}
\def\bG{\mathbf G}
\def\bI{\mathbf I}
\def\bE{\mathbf E}
\def\bP{\mathbf P}
\def\bfK{\mathbf K}
\def\bN{\mathbf N}
\def\bM{\mathbf M}
\def\bfM{\mathbf M}
\def\bfU{\mathbf U}
\def\bfT{{\mathbf T}}
\def\bfL{\mathbf L}
\def\bda{\mathbf a}
\def\bff{\mathbf f}
\def\bdh{\mathbf h}
\def\bdg{\mathbf g}
\def\bdx{\mathbf x}
\def\bdy{\mathbf y}
\def\bdp{\mathbf p}
\def\bfi{\mathbf i}
\def\bfu{\mathbf u}
\def\bdw{\mathbf w}
\def\bdS{\mathbf S}
\def\bdd{\mathbf d}
\def\bdc{\mathbf c}
\def\bdn{\mathbf n}
\def\bF{\mathbf F}
\def\bD{\mathbf D}
\def\bW{\mathbf W}
\def\bfw{\mathbf w}

%boldsymbol
\def\bfEucJ{\boldsymbol{\EucJ}}
\def\bfeta{\boldsymbol{\eta}}
\def\bflambda{\boldsymbol{\lambda}}
\def\bfrho{\boldsymbol{\rho}}
\def\bfdelta{\boldsymbol{\delta}}
\def\bftheta{\boldsymbol{\theta}}
\def\bfxi{\boldsymbol{\xi}}
\def\bfal{\boldsymbol{\alpha}}
\def\bfvep{\boldsymbol{\varepsilon}}
\def\bfep{\boldsymbol{\ep}}
\def\bfDelta{\boldsymbol{\Delta}}
% mathscr
\def\sG{\mathscr G}
\def\sH{\mathscr H}
\def\sF{\mathscr F}
\def\sL{\mathscr L}
\def\sI{\mathscr I}
\def\sJ{\mathscr J}
\def\sC{\mathscr C}
\def\sX{\mathscr X}
\def\sM{\mathscr M}
\def\sA{\mathscr A}
\def\sV{\mathscr V}
\def\sK{\mathscr K}
\def\sN{\mathscr N}
\def\sD{\mathscr D}
\def\sU{\mathscr U}
\def\sR{\mathscr R}
\def\sB{\mathscr B}
\def\sO{\mathscr O}
\def\sS{\mathscr S}
\def\sP{\mathscr P}
\def\sW{{\mathscr W}}
\def\sT{\mathscr T}
% mathbb
\def\T{{\mathbb T}}
\def\V{\mathbb V} %p-adic modular forms
\def\bbM{\mathbb M}
\def\bbI{\mathbb I}
\def\bbX{\mathbb X}
\def\bbY{\mathbb Y}
\def\bbJ{\mathbb J}
\def\bbL{\mathbb L}
\def\bbS{\mathbb S}
\newcommand{\Z}{\mathbf Z}
\newcommand{\Q}{\mathbf Q}
\newcommand{\R}{\mathbf R}
\newcommand{\C}{\mathbf C}
%\newcommand{\D}{\mathbf D}    % pro algebraic torus
\newcommand{\A}{\mathbf A}    % for adele
\newcommand{\F}{\mathbb F}
\def\bbK{\mathbb K}
\def\bbE{{\mathbb E}}
\def\bbV{\mathbb V}
\def\bbH{\mathbb H}
\def\bbW{\mathbb W}

\def\bbmu{\boldsymbol{\mu}}


% mathfrak
\def\cond{{c}}
\def\gm{{\mathfrak m}}

\def\fraka{{\mathfrak a}}
\def\frakb{{\mathfrak b}}
\def\frakc{{\mathfrak c}}
\def\frakd{\mathfrak d}
\def\frakf{\mathfrak f}
\def\frakk{\mathfrak k}
\def\frakp{{\mathfrak p}}
\def\frakP{\mathfak P}
\def\frakq{\mathfrak q}
\def\frakr{\mathfrak r}
\def\frakt{\mathfrak t}
\def\frakg{\mathfrak g}
\def\frakm{\mathfrak m}
\def\frakn{\mathfrak n}
\def\frakl{\mathfrak l}
\def\frakP{\mathfrak P}
\def\frakF{{\mathfrak F}}
\def\frakE{\mathfrak E}
\def\frakL{{\mathfrak L}}
\def\frakD{\mathfrak D}
\def\frakM{\mathfrak M}
\def\frakG{{\mathfrak G}}
\def\frakh{\mathfrak h}
\def\frakH{{\mathfrak H}}
\def\frakV{\mathfrak V}
\def\frakI{\mathfrak I}
\def\frakA{\mathfrak A}
\def\frakB{\mathfrak B}
\def\frakC{{\mathfrak C}}
\def\frakJ{\mathfrak J}
\def\frakX{\mathfrak X}
\def\frako{\mathfrak o}
\def\frakQ{\mathfrak Q}
\def\fraks{\mathfrak s}
\def\frakR{\mathfrak R}
\def\frakS{\mathfrak S}
\def\frakW{\mathfrak W}
\def\frakN{\mathfrak N}
\def\il{\mathfrak i\frakl}
\def\fraki{\mathfrak i}
\def\frakz{\mathfrak z}
%\mathpzc
\def\pzcw{\mathpzc w}
\def\pzcv{\mathpzc v}


% one
\def\bfone{{\mathbf 1}}
\def\bfzero{\mathbf 0}
\def\one{\mathbf 1} %trivial character

% underline
\def\ulA{\ul{A}}
\def\ulV{\ul{V}}
\def\ulW{\ul{W}}
\def\ulx{\ul{x}}
\def\ulN{\ul{N}}
\def\ulz{\ul{z}}
\def\ula{\ul{a}}
\def\nv{{\underline n}}

\def\ollam{\bar{\lam}}

%widetilde
\def\wtcG{\widetilde{\cG}}
\def\wtG{\widetilde{G}}
\def\wtE{\widetilde{E}}

%widehat
\def\whG{\widehat{G}}
\def\whX{\widehat{\chi}}
\def\whE{\widehat{E}}

%*********bar
\def\Vbar{\ol{V}}
\def\xbar{\ol{x}}
\def\ibar{\bar{i}}
\def\abar{\bar{a}}
\def\Hbar{\ol{H}}
\def\Zhat{\widehat{\Z}}
\def\wbar{\bar{w}}
\def\cSbar{\ol{\cS}}
\def\vbar{\bar{v}}
\def\wbar{\ol{w}}
\def\zbar{\ol{z}}


%******************French words
\def\et{{\acute{e}t}}

%****************** long words
%\def\SHA{\mathrm{III}}
\def\ac{algebraically closed }
\def\dieu{Dieudonn\'{e} }
\def\ab{abelian variety }
\def\etale{{\'{e}tale }}
%\newcommand{\abs}{abelian varieties }
\def\ss{supersingular }
\def\Eisen{Eisenstein }
\def\pont{Pontryagin } % Pontryagin dual
\def\padic{\text{$p$-adic }}
\def\auto{\text{automorphic }}
\def\BS{Bruhat-Schwartz }
\def\GinKarp{\text{Gindikin-Karpelevi\v{c} }}
\def\Versch{\emph{Verschiebung }}
\def\Shord{\text{Schr\"{o}dinger }}
\def\Schordinger{\text{Schr\"{o}dinger }}
\def\SerreH{\text{Serre-Hochschild }}
\def\Teich{Teichm\"{u}ller }
\def\Neron{N\'{e}ron }
\def\Frob{\mathrm{Frob}}
% moduli notation
\def\mg{{\mathcal M}_g}
\def\agd{{\mathcal A}_{g,d}}
\def\Ag{\mathcal A}

% \cal, \frak, \mathbf.. check Math Sci.
% \mathcal, \mathfrak, \EuScript (euscript), \mathbb

% better notation
\newcommand{\per}{\bot}
\newcommand{\<}{\langle}   %\< is not defined yet.
\renewcommand{\>}{\rangle} %\> is already defined.
\def\then{\Rightarrow}
\def\oneone{\mbox{$\longleftrightarrow$}}  %\11 can't be used
\def\isoto{\stackrel{\sim}{\to}}
\def\isotoL{\stackrel{\sim}{\leftarrow}}
\def\surjto{\twoheadrightarrow}
\def\imply{\Rightarrow}
\def\ot{\otimes}
\def\boxt{\boxtimes}
\def\hookto{\hookrightarrow}
\def\longto{\longrightarrow}
\def\ol{\overline}  \nc{\opp}{\mathrm{opp}} \nc{\ul}{\underline}
\newcommand\bra[1]{[{#1}]}
%\nc{\embed}{\hookrightarrow}

%useful operators
\newcommand{\pair}[2]{\< #1, #2\>}
\newcommand{\bbpair}[2]{\<\!\<#1,#2\>\!\>}
\newcommand{\altpair}[2]{(#1,#2)}
\newcommand{\rpair}[2]{(#1,#2)}
\newcommand{\brpair}[2]{[ #1, #2]}
\newcommand{\pairing}{\pair{\,}{\,}}
\def\bbpairing{\bbpair{\,}{\,}}
\def\altpairing{\altpair{\,}{\,}}
\def\rpairing{\altpair{\,}{\,}}
\def\brpairing{\brpair{\,}{\,}}
\newcommand{\defil}[2]{{#1}_1\supset {#1}_2\supset\dots\supset {#1}_{#2}}
\newcommand{\defilo}[2]{{#1}_0\supset {#1}_1\supset\dots\supset {#1}_{#2}}
\newcommand{\infil}[2]{{#1}_1\subset {#1}_2\subset\dots\subset {#1}_{#2}}
\newcommand{\infilo}[2]{{#1}_1\subset {#1}_1\subset\dots\subset
  {#1}_{#2}}
% never number appeared in the newcommand name!

\newcommand{\stackunder}[2]{\raisebox{-1ex}{$\stackrel{\textstyle
#1}{\scriptstyle #2}$}}


%XY matrix notation
\def\XYmatrix{\xymatrix@M=8pt} % make \xymatrix not too cluttered
\def\ncmd{\newcommand}
\ncmd{\xysubset}[1][r]{\ar@<-2.5pt>@{^(-}[#1]\ar@<2.5pt>@{_(-}[#1]}
\ncmd{\XYmatrixc}[1]{\vcenter{\XYmatrix{#1}}}
\ncmd{\xyto}[1][r]{\ar@{->}[#1]}
\ncmd{\xyinj}[1][r]{\ar@{^(->}[#1]}
\ncmd{\xysurj}[1][r]{\ar@{->>}[#1]}
\ncmd{\xyline}[1][r]{\ar@{-}[#1]}
\ncmd{\xydotsto}[1][r]{\ar@{.>}[#1]}
\ncmd{\xydots}[1][r]{\ar@{.}[#1]}
\ncmd{\xyleadsto}[1][r]{\ar@{~>}[#1]}
\ncmd{\xyeq}[1][r]{\ar@{=}[#1]} \ncmd{\xyequal}[1][r]{\ar@{=}[#1]}
\ncmd{\xyequals}[1][r]{\ar@{=}[#1]}
\ncmd{\xymapsto}[1][r]{l\ar@{|->}[#1]}\ncmd{\xyimplies}[1][r]{\ar@{=>}[#1]}
\ncmd{\xyiso}{\ar[r]_-{\sim}}
\def\injxy{\ar@{^(->}}

%*************************Matrices
\newcommand{\Cln}[3]{\bbmx #1\\#2\\#3 \ebmx}

\newcommand{\mx}[4]{\begin{array}{cc}{#1}&
 {#2}\\{#3}&{#4}\end{array}}
\newcommand{\MX}[4]{\begin{bmatrix}
{#1}& {#2}\\
{#3}&{#4}\end{bmatrix} }

\newcommand{\pMX}[4]{\begin{pmatrix}
{#1}& {#2}\\
{#3}&{#4}\end{pmatrix} }

\newcommand{\bMX}[4]{\left[\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}\end{matrix}\right]}

 \newcommand{\DII}[2]{\begin{bmatrix}{#1}&0
 \\0&{#2}\end{bmatrix}}
 \newcommand{\pDII}[2]{\begin{pmatrix}{#1}&0
 \\0&{#2}\end{pmatrix}}

\newcommand{\DIII}[3]{\begin{bmatrix}{#1}&&\\
&{#2}&\\
&&{#3}\end{bmatrix}}

\newcommand{\UPIII}[3]{\begin{bmatrix}1&{#1}&{#2}\\
&1&{#3}\\
&&1\end{bmatrix}}

\newcommand{\cln}[2]{\left[\begin{matrix}
  {#1} \\
  {#2}\\
\end{matrix}\right]
}
\newcommand{\xcln}[2]{\begin{matrix}
  {#1} \\
  {#2}\\
\end{matrix}
}
\newcommand{\xrow}[2]{\begin{matrix}
  {#1} &{#2}
\end{matrix}
}
\newcommand{\ADIII}[3]{\begin{bmatrix}
   &  &{#1}  \\
   &{#2} & \\
   {#3}&  &  \\
\end{bmatrix}}

\newcommand{\DIV}[4]{\begin{bmatrix}
{#1}&&&\\
&{#2}&&\\
&&{#3}&\\
&&&{#4}
\end{bmatrix}}



%Metaplectic group
\newcommand\Meta[2]{\left({#1},{#2}\right)}
\def\tj{\tilde{j}}
\def\wtSL{\widetilde{\SL}}
\newcommand{\seesaw}[4]{{#1}\ar@{-}[rd]\ar@{-}[d]&{#2}\ar@{-}[d]\\
{#3}\ar@{-}[ru]&{#4}}

%Duals
\newcommand\dual[1]{{#1}^{\!\vee}} %Dual
\newcommand\Pdual[1]{{#1}^*} %Pontragin dual
\newcommand\Cdual[2]{{#1}^D} %Cartier dual


% *** ENGLISH ABBREVIATIONS ****************************************

% Some words
\def\by{\text{ by }}
\def\where{\text{ where }}
\def\ie{i.e. }
\def\eg{\mbox{{\it e.g.} }}
\def\etc{\mbox{{\it et cetera} }}
\def\cf{\mbox{{\it cf.} }}
\def\loccit{\mbox{{\it loc.cit.} }}
\def\opcit{\mbox{{\it op.cit.} }}
\def\can{{can}}
\def\etal{\mbox{{ et al.}}}
\def\resp{resp.$\,$}


%\renewcommand{\O}{\cO}
\def\wht#1{\widehat{#1}}
\def\Cyc{{\langle\varepsilon\rangle}}%universal deformation of cyclotomoic character
%\newcommand{\deform}[1]{\tilde{{#1}}}

%Category
\def\ENS{\mathfrak E\mathfrak n\mathfrak s}
\def\SCH{\mathfrak S\mathfrak c\mathfrak h}

% for extending arrows
\def\ext{\rule[.5ex]{5mm}{.1mm}}
\def\EXt{\rule[.5ex]{10mm}{.1mm}}
\def\back{\!\!\!}
\def\Back{\back\back}
% right surjective maps
\def\onsuffix{\longrightarrow\back\back\!\rightarrow}

\def\maponR{\smash{\mathop{\onsuffix}}}
\def\maponRR{\smash{\mathop{\ext\back\onsuffix}}}
\def\maponRRR{\smash{\mathop{\EXt\back\onsuffix}}}

\def\MaponR#1#2{\smash{\mathop{\onsuffix}\limits^{#1}_{#2}}}
\def\MaponRR#1#2{\smash{\mathop{\ext\back\onsuffix}\limits^{#1}_{#2}}}
\def\MaponRRR#1#2{\smash{\mathop{\EXt\back\onsuffix}\limits^{#1}_{#2}}}

% right maps
\def\mapR{\smash{\mathop{\longrightarrow}}}
\def\mapRR{\smash{\mathop{\ext\back\longrightarrow}}}
\def\mapRRR{\smash{\mathop{\Ext\back\longrightarrow}}}

\def\MapR#1#2{\smash{\mathop{\longrightarrow}\limits^{#1}_{#2}}}
\def\MapRR#1#2{\smash{\mathop{\ext\back\longrightarrow}\limits^{#1}_{#2}}}
\def\MapRRR#1#2{\smash{\mathop{\Ext\back\longrightarrow}\limits^{#1}_{#2}}}

% right injective maps
\def\inprefix{\mbox{\raisebox{1mm}{\tiny $\subset$}}\!\!}

\def\mapinR{\smash{\mathop{\inprefix\!\!\longrightarrow}}}
\def\mapinRR{\smash{\mathop{\inprefix\ext\back\longrightarrow}}}
\def\mapinRRR{\smash{\mathop{\inprefix\Ext\back\longrightarrow}}}

\def\MapinR#1#2{\smash{\mathop{\inprefix\!\!\longrightarrow}\limits^{#1}_{#2}}}
\def\MapinRR#1#2{\smash{\mathop{\inprefix\ext\back\longrightarrow}\limits^{#1}_{#2}}}
\def\MapinRRR#1#2{\smash{\mathop{\inprefix\Ext\back\longrightarrow}\limits^{#1}_{#2}}}

% exact sequence
\newcommand{\exact}[3]{
0\mapR{#1}\mapR{#2}\mapR{#3}\mapR 0 }
\newcommand{\Exact}[5]{
0\mapR{#1}\MapR{#2}{} {#3}\MapR{#4}{} {#5}\mapR 0 }

\newcommand{\edit}[1]{\footnote{#1}\marginpar{\hfill {\sf\thefootnote}}}
\newcommand{\todo}[1]{\noindent$\bullet$ {\small \textsf{#1}} $\bullet$\\}
\newcommand{\done}[1]{\noindent {\small \textsf{Done: #1}}\\}
\newcommand{\danger}[1]{\marginpar{\small \textsl{#1}}}

% characteristic function of a set
\def\Ch{\mathrm{char}}
%\newcommand{\ch}{characteristic }
\def\ch{{\mathbb I}}

\def\hb#1{\hbox{ #1}}

%Local fields
\def\uf{\varpi} %uniformizer
\def\Abs{{|\!\cdot\!|}} %adelic absolute value
%\providecommand\abs[1]{\lvert{#1}\rvert}

% Control symbols
\newcommand{\npr}{\noindent }
\newcommand{\pr}{\indent }


% abbreviation
\def\Sg{{\varSigma}}  %%CM type
\def\Sgbar{\Sg^c}
\def\ndivides{\nmid}
\def\ndivide{\nmid}
\def\x{{\times}}
\def\xx{\,\times\,}
\def\tame{\mathrm{tame}}
\def\onehalf{{\frac{1}{2}}}
\def\e{\varepsilon} % episilon factor
\def\al{\alpha}
\def\Beta{\boldsymbol \beta}
\def\Lam{\Lambda}
\def\kap{\kappa}
\def\om{\omega}
\def\dirlim{\varinjlim}
\def\prolim{\varprojlim}
\def\iso{\simeq}
\def\con{\equiv}
\def\bksl{\backslash}
\newcommand\stt[1]{\left\{#1\right\}}
\def\ep{\epsilon}
\def\varep{\varepsilon}
\def\l{{\ell}}
\def\pd{\partial}
\def\lam{\lambda}
\def\AI{\textrm{AI}} % automotphic induction
\def\pii{\pi i}
\def\hot{\widehat{\ot}}
\def\half{\frac{1}{2}}
\def\Ups{\Upsilon}
\def\cpd{2\pi i}
\def\vep{\varepsilon}
\def\ka{\kappa}
\def\sg{\sigma}
\def\vp{\varphi}
\def\disjoint{\sqcup}
\def\bigot{\bigotimes}
\def\Pol{\mathrm{Pol}}
\def\smid{\,|}

%Symbol for measures
\def\dx{{\rm d}^\x}
\def\dxx{{\rm d}^\x x}
\def\dxv{dx_v}
\def\dxp{dx_p}
\def\dd{{\rm d}}

% ideles and adeles
\def\Adele#1{#1(\Q)\bksl #1(\A)}
\def\idele{\A^\times}
\def\AFf{\A_{\cF,f}}
\def\AKf{\A_{\cK,f}}
\def\AF{\A_\cF}
\def\AK{\A_\cK}
\def\setp{{(p)}}
\def\setinfp{{(\infty,p)}}
\def\setinf{{(\infty)}}
\def\bbox{{(\Box)}}

\newcommand{\powerseries}[1]{\llbracket{#1}\rrbracket}
\newcommand{\formal}[1]{\widehat{#1}}
\renewcommand\pmod[1]{\,(\mbox{mod }{#1})}
\renewcommand\mod[1]{\,\mbox{mod }{#1}}
\newcommand\PD[1]{\frac{\partial}{\partial{#1}}}
%\newcommand\DD[2]{\frac{\partial{#1}}{\partial{#2}}}
\renewcommand\Re{\text{Re}\,}
\newcommand\Dmd[1]{\left<{#1}\right>} %Diamond operator
\def\vphi{\varphi}
\def\Her{\EucH} %Hermitian matrix
\def\Cp{\C_p}
\def\inert{{\mathrm{inert}}}
\def\ram{{\mathrm{ram}}}
\def\split{{\mathrm{split}}}
\def\alg{\mathrm{alg}} 
\def\Qq{\Q_q} 
\def\pmq{q}
\def\cond{{\rm cond}}



==> SO(5)xGL(2)/mathdots/README <==
This is the mathdots package, version 0.9.
Copyright 2001--2014, Daniel H. Luecking

License:
=======
Mathdots may be distributed and/or modified under the conditions of the
LaTeX Project Public License, either version 1.3c of this license or (at
your option) any later version. The latest version of this license is in
   <http://www.latex-project.org/lppl.txt>
and version 1.3c or later is part of all distributions of LaTeX dated
2008/05/04 or later.

Mathdots has maintenance status "author-maintained". The Current
Maintainer is Daniel H. Luecking. The Base Interpreters associated with
mathdots are plain TeX and LaTeX

Purpose:
=======
This package changes the basic LaTeX and plain TeX commands \ddots and
\vdots so that they properly change size when font sizes change, and
when they are used in superscripts and subscripts. It also adds the
command \iddots (for inverse diagonal dots) which slants the opposite
way from \ddots.

In addition, if it detects amsmath in LaTeX (or AMSTeX in plain TeX) it
defines improved versions of the \dddot and \ddddot commands that place
three and four dots on a math symbol (similar to the math accent
commands \dot and \ddot). These also are arranged to change size
correctly and some placement bugs are corrected.

Other (minor) improvements: the commands \vdots, \ddots and \iddots
select the dot from the math fonts instead of the text fonts, so they
always match math punctuation dots. The \dddot and \ddddot commands
select the accent dot (same one placed by \dot).

File list:

README          This file
mathdots.dtx    The code
mathdots.pdf    The manual
mathdots.ins    unpacking script
mdotest.tex     LaTeX test file
plmdotest.tex   Plain TeX test file (requires loading amstex.tex and the
                and something to define the commands \eightpoint,
                \ninepoint, \tenpoint and \twelvepoint)

Installation:

Run tex or latex on mathdots.ins to unpack the files. Copy mathdots.tex
where tex will find it and mathdots.sty where latex will find it. Copy
the remaining files to your documentation area.

Daniel H. Luecking, \luecking \at \uark \dot \edu



==> SO(5)xGL(2)/mathdots/plmdotest.tex <==
\input amstex
\input mathdots

\eightpoint
eightpoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\ninepoint
ninepoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\tenpoint
tenpoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\twelvepoint
twelvepoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\enddocument\end


==> SO(5)xGL(2)/mnsymbol/README <==
MnSymbol is a symbol font designed to be used in conjunction with Adobe
MinionPro.

All files in this archive are in the public domain.

WARNING
=======

This version includes a bugfix that causes incompatibilities with
previous versions. The symbols

  \...harpoonup and \...harpoondown

are now called

  \...harpoonccw and \...harpooncw

(This was needed for compatibility with amsfonts.sty.)

INSTALLATION
============

To install the fonts:

(0) If you have already a version of MnSymbol installed, delete the old
TFM and PK files.

(1) Run

  $ cd tex
  $ latex MnSymbol.ins

and copy the resulting file MnSymbol.sty to

   .../texmf/tex/latex/MnSymbol/MnSymbol.sty

(2) Copy all files in the "source" directory into the directory

   .../texmf/fonts/source/public/MnSymbol/

(3) Copy the documentation (MnSymbol.ps, MnSymbol.pdf, README) into the
directory

   .../texmf/doc/latex/MnSymbol/

(4) To install the PostScript fonts (courtesy of Michael Zedler) copy

  o enc/MnSymbol.map into .../texmf/fonts/map/dvips/MnSymbol
  o enc/*.enc        into .../texmf/fonts/enc/dvips/MnSymbol
  o pfb/*.pfb        into .../texmf/fonts/type1/public/MnSymbol

(These fonts are not strictly necessary but recommended.)

(5) You can copy the files in the "tfm" directory to

   .../texmf/fonts/tfm/public/MnSymbol

This is optional since these files can be generated automatically.
But it saves some time.

(6) Regenerate the file database:

  $ mktexlsr

If you installed the PostScript fonts you also need to run updmap or
updmap-sys to make them available:

  $ updmap-sys --enable MixedMap MnSymbol.map

(7) Happy TeXing.

Achim Blumensath


==> SO(5)xGL(2)/tikz-cd/tikzlibrarycd.code.tex <==
% tikzlibrarycd.code.tex [2018/11/19 v0.9f Commutative diagrams with TikZ]
%
% Copyright 2011, 2012, 2014, 2018 by Augusto Stoffel
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.

\usetikzlibrary{matrix,quotes,arrows.meta}

\newif\iftikzcd@mathmode

\def\tikzcdset{\pgfqkeys{/tikz/commutative diagrams}}

\tikzcdset{
  arrows/.code={\tikzcdset{every arrow/.append style={#1}}},
  labels/.code={\tikzcdset{every label/.append style={#1}}},
  cells/.code={\tikzcdset{every cell/.append style={#1}}},
  diagrams/.code={\tikzcdset{every diagram/.append style={#1}}},
  execute before arrows/.code={%
    \expandafter\def%
    \expandafter\tikzcd@before@paths@hook%
    \expandafter{\tikzcd@before@paths@hook#1}},
  to/.code={\tikzcd@setarrowend\tikzcd@ar@target{#1}},
  from/.code={\tikzcd@setarrowend\tikzcd@ar@start{#1}},
  shorten/.style={
    /tikz/shorten <=#1,
    /tikz/shorten >=#1},
  description/.style={
    /tikz/anchor=center,
    /tikz/fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color}},
  marking/.style={
    /tikz/font=,
    /tikz/sloped,
    /tikz/shape=asymmetrical rectangle,
    /tikz/anchor=center},
  phantom/.style={
    /tikz/draw=none,
    /tikz/commutative diagrams/labels={
      /tikz/font=,
      /tikz/anchor=center}},
  crossing over/.style={
    /tikz/preaction={
      /tikz/draw=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
      /tikz/arrows=-,
      /tikz/line width=\pgfkeysvalueof{/tikz/commutative diagrams/crossing over clearance}}},
  cramped/.code={\tikzcdset{
    every matrix/.append style={inner sep=+-0.3em},
    every cell/.append style={inner sep=+0.3em}}},
  row sep/.code={\tikzcd@sep{row}{#1}},
  column sep/.code={\tikzcd@sep{column}{#1}},
  sep/.code={\tikzcdset{row sep={#1},column sep={#1}}},
  math mode/.is if=tikzcd@mathmode,
  arrow style/.is choice}

\def\tikzcd@sep#1#2{%
  \pgfkeysifdefined{/tikz/commutative diagrams/#1 sep/#2}%
    {\pgfkeysgetvalue{/tikz/commutative diagrams/#1 sep/#2}\tikzcd@temp%
     \pgfkeysalso{/tikz/#1 sep/.expand once=\tikzcd@temp}}%
    {\pgfkeysalso{/tikz/#1 sep={#2}}}}

\def\tikzcd@setarrowend#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@\tikzcdmatrixname-#2}%
    {%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp#2\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef#1{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \def#1{#2}%
      \fi%
    }{%
      \def#1{\tikzcdmatrixname-#2}%
    }}
    
% The unknown key handler and direction argument parser
\tikzcdset{
  .unknown/.code={%
    \ifpgfkeysaddeddefaultpath%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp\pgfkeyscurrentname\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef\tikzcd@ar@target{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \pgfqkeys{/tikz}{\pgfkeyscurrentname={#1}}%
      \fi%
    \else%
      \def\pgfutilnext{\pgfkeysvalueof{/handlers/.unknown/.@cmd}#1\pgfeov}\pgfutilnext%
    \fi}}

\def\tikzcd@parse#1{% parser for arrow direction argument
  \ifx#1r\advance\c@pgf@countb by1\else%
   \ifx#1d\advance\c@pgf@counta by1\else%
    \ifx#1l\advance\c@pgf@countb by-1\else%
     \ifx#1u\advance\c@pgf@counta by-1\else%
      \ifx#1\relax\let\tikzcd@temp\pgfutil@empty%
       \else\let\tikzcd@temp\pgfutil@gobble@until@relax\fi\fi\fi\fi\fi%
  \tikzcd@temp}

% The `tikzcd' environment
\def\tikzcd{%
  \iffalse{\fi\ifnum0=`}\fi% standard trick to allow nesting of tabular-like environments (cf. the tabularx manual)
  \pgfutil@ifnextchar&% if we get an & here, it will be returned with the wrong catcode to the input stream
    {\expandafter\tikzcd@@\expandafter\pgfmatrixnextcell\pgfutil@gobble}%
    {\tikzcd@@}}

\def\tikzcd@@{\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@}{\tikzcd@[]}}

\def\tikzcd@[#1]{%
  \tikzpicture[/tikz/commutative diagrams/.cd,every diagram,#1]%
  \ifx\arrow\tikzcd@arrow%
    \pgfutil@packageerror{tikz-cd}{Diagrams cannot be nested}{}%
  \fi%
  \let\arrow\tikzcd@arrow%
  \let\ar\tikzcd@arrow%
  \def\rar{\tikzcd@xar{r}}%
  \def\lar{\tikzcd@xar{l}}%
  \def\dar{\tikzcd@xar{d}}%
  \def\uar{\tikzcd@xar{u}}%
  \def\urar{\tikzcd@xar{ur}}%
  \def\ular{\tikzcd@xar{ul}}%
  \def\drar{\tikzcd@xar{dr}}%
  \def\dlar{\tikzcd@xar{dl}}%
  \global\let\tikzcd@savedpaths\pgfutil@empty%
  \matrix[%
    /tikz/matrix of \iftikzcd@mathmode math \fi nodes,%
    /tikz/every cell/.append code={\tikzcdset{every cell}},%
    /tikz/commutative diagrams/.cd,every matrix]%
  \bgroup}

\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths%
  \endgroup%
  \endtikzpicture%
  \ifnum0=`{}\fi}

% The arrow commands
\def\tikzcd@arrow{%
  \relax% this was added to avoid errors when a cell starts with \arrow, but it seems unnecessary now
  \edef\tikzcd@temp{%
    \noexpand\def\noexpand\tikzcd@currentcolumn{\the\pgfmatrixcurrentcolumn}%
    \noexpand\def\noexpand\tikzcd@currentrow{\the\pgfmatrixcurrentrow}%
    \noexpand\def\noexpand\tikzcd@lineno{\the\inputlineno}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@savedpaths\expandafter{\tikzcd@temp}%
  \pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@arrow}{\tikzcd@ar@old[]}}

\def\tikzcd@@arrow[#1]{\pgfutil@ifnextchar\bgroup{\tikzcd@ar@old[#1]}{\tikzcd@ar@new[#1]}}

\def\tikzcd@ar@new[#1]{% new syntax
  \pgfutil@g@addto@macro\tikzcd@savedpaths{%
    \path[/tikz/commutative diagrams/.cd,every arrow,#1]%
    (\tikzcd@ar@start\tikzcd@startanchor) to (\tikzcd@ar@target\tikzcd@endanchor); }}

\def\tikzcd@ar@old[#1]#2{% old syntax
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{to={#2},#1}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{to={#2},#1}[]}%
      {\tikzcd@ar@new[to={#2},#1]}}}

\def\tikzcd@ar@getlabel#1[#2]#3{%
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{#1,"{#3}"{#2}}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{#1,"{#3}"{#2}}[]}%
      {\tikzcd@ar@new[#1,"{#3}"{#2}]}}}

\def\tikzcd@xar#1{\relax\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@xar{#1}}{\tikzcd@arrow[]{#1}}}
\def\tikzcd@@xar#1[#2]{\tikzcd@arrow[#2]{#1}}

\def\tikzcd@handle@shortcuts@next{% expand next macro using standard catcodes
  \iftikz@handle@active@code%
    \begingroup%
      \tikz@switchoff@shorthands\expandafter%
    \endgroup\expandafter%
  \fi}

\def\tikzcd@ar@target{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}
\def\tikzcd@ar@start{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}

\def\tikzcd@forward@quotes#1{\tikzset{every to/.append style={#1}}}

\let\tikzcd@before@paths@hook\pgfutil@empty

% `start anchor', `end anchor', and `shift' keys
\def\tikzcd@setanchor#1[#2]#3\relax{%
  \ifx\relax#2\relax\else%
    \tikzcdset{@#1transform/.append style={#2},@shiftabletopath}%
  \fi%
  \ifx\relax#3\relax%
    \pgfutil@namelet{tikzcd@#1anchor}{pgfutil@empty}%
  \else%
    \pgfutil@namedef{tikzcd@#1anchor}{.#3}%
  \fi}

\tikzcdset{
  @shiftabletopath/.style={
    /tikz/execute at begin to={%
      \begingroup%
        \def\tikz@tonodes{coordinate[pos=0,commutative diagrams/@starttransform/.try](tikzcd@nodea) %
                          coordinate[pos=1,commutative diagrams/@endtransform/.try](tikzcd@nodeb)}%
        \path (\tikztostart) \tikz@to@path;%
      \endgroup%
      \def\tikztostart{tikzcd@nodea}%
      \def\tikztotarget{tikzcd@nodeb}%
      \tikzset{insert path={(tikzcd@nodea)}}},
    /tikz/commutative diagrams/@shiftabletopath/.code={}},
  start anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{start}}{\tikzcd@setanchor{start}[]}#1\relax},%]
  end anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{end}}{\tikzcd@setanchor{end}[]}#1\relax},%]
  start anchor=,
  end anchor=,
  shift left/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/execute at begin to={%
      \pgfpointnormalised{%
        \pgfpointdiff{\pgfpointanchor{tikzcd@nodeb}{center}}{\pgfpointanchor{tikzcd@nodea}{center}}}%
      \pgfgetlastxy{\tikzcd@x}{\tikzcd@y}%
      \pgfmathparse{#1}%
      \ifpgfmathunitsdeclared\else
        \pgfmathparse{\pgfmathresult*\pgfkeysvalueof{/tikz/commutative diagrams/shift left/.@def}}
      \fi
      \coordinate (tikzcd@nodea) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodea);%
      \coordinate (tikzcd@nodeb) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodeb);%
      \tikzset{insert path={(tikzcd@nodea)}}}},
  shift right/.style={
    /tikz/commutative diagrams/shift left={-(#1)}},
  transform nodes/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/commutative diagrams/@starttransform/.append style={#1},
    /tikz/commutative diagrams/@endtransform/.append style={#1}},
  shift/.style={
    /tikz/shift={#1},% we need this for labels to receive a shift
    /tikz/commutative diagrams/transform nodes={/tikz/shift={#1}}},
  xshift/.style={
    /tikz/xshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/xshift={#1}}},
  yshift/.style={
    /tikz/yshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/yshift={#1}}}}

% pgfmath functions to obtain math fontdimens
\pgfutil@ifluatex

  \directlua{tex.enableprimitives('tikzcd@', {'Umathaxis', 'Umathfractionrule'})}

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\tikzcd@Umathaxis\textstyle%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\tikzcd@Umathfractionrule\textstyle%
    \endgroup}

\else% if using (pdf)tex

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\fontdimen22\textfont2%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\fontdimen8\textfont3%
    \endgroup}

\fi

% The shape used inside matrices
\pgfdeclareshape{asymmetrical rectangle} {
  \inheritsavedanchors[from={rectangle}]
  \inheritanchor[from={rectangle}]{base}
  \inheritanchor[from={rectangle}]{north}
  \inheritanchor[from={rectangle}]{south}
  \inheritanchor[from={rectangle}]{base west}
  \inheritanchor[from={rectangle}]{north west}
  \inheritanchor[from={rectangle}]{south west}
  \inheritanchor[from={rectangle}]{base east}
  \inheritanchor[from={rectangle}]{north east}
  \inheritanchor[from={rectangle}]{south east}
  \inheritanchor[from={rectangle}]{mid}
  \inheritanchor[from={rectangle}]{mid west}
  \inheritanchor[from={rectangle}]{mid east}
  \inheritbackgroundpath[from={rectangle}]
  \anchor{center}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{west}{\pgf@anchor@rectangle@west\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{east}{\pgf@anchor@rectangle@east\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{real center}{\pgf@anchor@rectangle@center}
  \anchor{real west}{\pgf@anchor@rectangle@west}
  \anchor{real east}{\pgf@anchor@rectangle@east}
  \anchorborder{%
    \pgfmathsetlength\pgfutil@tempdima%
      {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \ifdim\pgf@yb>0pt%
      \northeast%
      \pgf@yc=\pgf@y%
      \advance\pgf@yc by-\pgfutil@tempdima%
    \else%
      \southwest%
      \pgf@yc=-\pgf@y%
      \advance\pgf@yc by\pgfutil@tempdima%
    \fi
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgfutil@tempdima%
  }%
}%

% Computer modern arrow tips
\pgfkeys{
  cm to/.tip={Computer Modern Rightarrow[length=+0pt 6.2]},
  cm bold to/.tip={cm to[scale=0.667]},
  cm double to/.tip={cm to[sep=+0pt -2.6]cm to},
  cm bar/.tip={Bar[width=+0pt 8.2 0.89,line cap=round]},
  cm left hook/.tip={Hooks[width=+0pt 10.8,length=+0pt 3.6,harpoon,line cap=round]},
  cm implies/.tip={Implies},
  cm left to/.tip={cm to[left]},
  cm right to/.tip={cm to[right]},
  cm right hook/.tip={cm left hook[swap]},
  cm to reversed/.tip={cm to[reversed]},
  cm */.tip={Circle[length=+0pt 7.6]},
  cm o/.tip={cm *[open]},
  cm |/.tip={cm bar}}%|

% The `Glyph' meta arrow tip
\pgfqkeys{/pgf/arrow keys}{
  glyph math command/.code={% if csname #1 is undefined, we want it to remain so
    \pgfarrowsaddtooptions{\def\tikzcd@glyph{$\begingroup\expandafter\endgroup\csname #1\endcsname$}}},
  glyph axis/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@axis{#1}}},
  glyph length/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@len{#1}}},
  glyph shorten/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@shorten{#1}}}}

\pgfdeclarearrow{
  name=Glyph,
  cache=false,
  bending mode=none,
  parameters={\tikzcd@glyph@len,\tikzcd@glyph@shorten},
  setup code={%
    \pgfarrowssettipend{\tikzcd@glyph@len\advance\pgf@x by\tikzcd@glyph@shorten}},
  defaults={
    glyph axis=axis_height,
    glyph length=+0.9ex,
    glyph shorten=+-0.1ex},
  drawing code={%
    \pgfpathrectangle{\pgfpoint{+0pt}{+-1ex}}{\pgfpoint{+\tikzcd@glyph@len}{+2ex}}%
    \pgfusepathqclip%
    \pgftransformxshift{+\tikzcd@glyph@len}%
    \pgftransformyshift{+-\tikzcd@glyph@axis}%
    \pgftext[right,base]{\tikzcd@glyph}}}

% Arrow tip selection styles
\tikzcdset{
  double line/.code={\tikzset{%
    double equal sign distance,
    double=\pgfkeysvalueof{/tikz/commutative diagrams/background color}}},
  dashed/.style={/tikz/dash pattern={on 7\pgflinewidth off 4\pgflinewidth}},
  tikzcd to/.tip={cm to},
  tikzcd bar/.tip={cm bar},
  tikzcd left hook/.tip={cm left hook},
  tikzcd double to/.tip={cm double to},
  tikzcd implies/.tip={Implies},
  tikzcd right hook/.tip={tikzcd left hook[swap]},
  tikzcd left to/.tip={tikzcd to[harpoon]},
  tikzcd right to/.tip={tikzcd left to[swap]},
  tikzcd to reversed/.tip={tikzcd to[reversed]},
  tikzcd cap/.tip={},
  tikzcd implies cap/.tip={},
  tikzcd implies bar/.tip={tikzcd bar},
  no tail/.code={\pgfsetarrowsstart{tikzcd cap}},
  to head/.code={\pgfsetarrowsend{tikzcd to}},
  maps to/.code={\pgfsetarrowsstart{tikzcd bar}},
  hook/.code={\pgfsetarrowsstart{tikzcd right hook}},
  hook'/.code={\pgfsetarrowsstart{tikzcd left hook}},
  harpoon/.code={\pgfsetarrowsend{tikzcd left to}},
  harpoon'/.code={\pgfsetarrowsend{tikzcd right to}},
  two heads/.code={\pgfsetarrowsend{tikzcd double to}},
  tail/.code={\pgfsetarrowsstart{tikzcd to reversed}},
  rightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd to}},
  Rightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies}},
  leftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd cap}},
  Leftarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies cap}},
  leftrightarrow/.code={\pgfsetarrows{tikzcd to-tikzcd to}},
  Leftrightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies}},
  mapsto/.code={\pgfsetarrows{tikzcd bar-tikzcd to}},
  mapsfrom/.code={\pgfsetarrows{tikzcd to-tikzcd bar}},
  Mapsto/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies bar-tikzcd implies}},
  Mapsfrom/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies bar}},
  hookrightarrow/.code={\pgfsetarrows{tikzcd right hook-tikzcd to}},
  hookleftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd left hook}},
  rightharpoonup/.code={\pgfsetarrows{tikzcd cap-tikzcd left to}},
  rightharpoondown/.code={\pgfsetarrows{tikzcd cap-tikzcd right to}},
  leftharpoonup/.code={\pgfsetarrows{tikzcd right to-tikzcd cap}},
  leftharpoondown/.code={\pgfsetarrows{tikzcd left to-tikzcd cap}},
  rightarrowtail/.code={\pgfsetarrows{tikzcd to reversed-tikzcd to}},
  leftarrowtail/.code={\pgfsetarrows{tikzcd to-tikzcd to reversed}},
  twoheadrightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd double to}},
  twoheadleftarrow/.code={\pgfsetarrows{tikzcd double to-tikzcd cap}},
  no head/.code={\pgfsetarrowsend{tikzcd cap}},
  dash/.code={\pgfsetarrows{tikzcd cap-tikzcd cap}},
  dashrightarrow/.code={\tikzcdset{rightarrow,dashed}},
  dashleftarrow/.code={\tikzcdset{leftarrow,dashed}},
  equal/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies cap}},
  equals/.code={\tikzcdset{equal}},
  rightsquigarrow/.code={\tikzcdset{rightarrow,squiggly}},
  leftsquigarrow/.code={\tikzcdset{leftarrow,squiggly}},
  leftrightsquigarrow/.code={\tikzcdset{leftrightarrow,squiggly}},
  squiggly/.code={%
    \pgfutil@ifundefined{tikz@library@decorations.pathmorphing@loaded}%
      {\pgfutil@packageerror{tikz-cd}{You need to say %
      \string\usetikzlibrary{decorations.pathmorphing} to use squiggly arrows}{}}{}%
    \pgfkeysalso{
      /tikz/decorate,
      /tikz/decoration={
        zigzag,
        segment length=9.25\pgflinewidth,
        amplitude=1.9\pgflinewidth,
        post=lineto, post length=6\pgflinewidth,
        pre=lineto, pre length=6\pgflinewidth,
        #1}}}}

% The `Latin Modern' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/Latin Modern}{%
  \tikzcdset{
    tikzcd bar/.tip={Bar[width=+0pt 12 .992,line cap=round]},
    tikzcd left hook/.tip={Hooks[width=+0pt 15,length=+0pt 4.2,arc=190,harpoon,line cap=round]}}}

% The `tikz' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/tikz}{%
  \tikzcdset{
    tikzcd to/.tip={>},
    tikzcd bar/.tip={Bar[width=+3pt 4 0.9]},
    tikzcd left hook/.tip={Hooks[harpoon]},
    tikzcd double to/.tip={tikzcd to[]tikzcd to}}}

% The `math font' arrow style
%
% If your font does not define the command \mapsfrom, do so by saying
%   \def\mapsfrom{\pgfpicture\pgfsetbaseline{+0pt}\pgftransformxscale{-1}\pgftext[base]{$\mapsto$}\endpgfpicture}
%
% The method used to guess the correct value of `double distance'
% inside the `double line' style is not robust at all.  If it fails,
% set
%   \tikzcdset{double line/.append style={double distance=2*rule_thickness}}
% and find the correct value for `double distance' by trial and error
% (or measure the distance between the \Rightarrow stems in a font
% editor).
%
\pgfkeysdef{/tikz/commutative diagrams/arrow style/math font}{%
  \tikzcdset{
    tikzcd to/.tip={Glyph[glyph math command=rightarrow]},
    tikzcd cap/.tip={Glyph[glyph math command=leftarrow]},
    tikzcd to reversed/.tip={Glyph[glyph math command=leftarrowtail]},
    tikzcd bar/.tip={Glyph[glyph math command=mapsfrom]},
    tikzcd left hook/.tip={Glyph[glyph math command=hookleftarrow]},
    tikzcd right hook/.tip={Glyph[glyph math command=hookleftarrow, swap]},
    tikzcd implies/.tip={Glyph[glyph math command=Rightarrow, glyph length=1.2ex]},
    tikzcd implies cap/.tip={Glyph[glyph math command=Leftarrow]},
    tikzcd implies bar/.tip={Glyph[glyph math command=Mapsfrom]},
    tikzcd double to/.tip={Glyph[glyph math command=twoheadrightarrow, glyph length=1.4ex]},
    tikzcd left to/.tip={Glyph[glyph math command=rightharpoonup]},
    tikzcd right to/.tip={Glyph[glyph math command=rightharpoonup,swap]},
    double line/.append code={\tikzset{double distance={2*(height("$=$")-axis_height-rule_thickness)}}},
    dashed/.code={\tikzset{dash pattern=on 0.8ex off 0.4ex, dash phase=0.8ex}},
    squiggly/.default={pre length=1ex, post length=1ex}}}

% Default settings
\tikzcdset{
  every arrow/.style={
    /tikz/draw,
    /tikz/line width=rule_thickness,
    /tikz/commutative diagrams/rightarrow},
  every label/.style={
    /tikz/auto,
    /tikz/font=\everymath\expandafter{\the\everymath\scriptstyle},
    /tikz/inner sep=+0.5ex},
  every cell/.style={
    /tikz/shape={asymmetrical rectangle},
    /tikz/inner xsep=+1ex,
    /tikz/inner ysep=+0.85ex},
  every matrix/.style={/tikz/inner sep=+0pt},
  every diagram/.style={
    /tikz/commutative diagrams/row sep=normal,
    /tikz/commutative diagrams/column sep=normal,
    /tikz/baseline=+0pt},
  1-row diagram/.style={/tikz/baseline/.expanded=(\tikzcdmatrixname.base)},
  math mode=true,
  center yshift/.initial=axis_height,
  row sep/huge/.initial=+3.6em,
  row sep/large/.initial=+2.7em,
  row sep/normal/.initial=+1.8em,
  row sep/scriptsize/.initial=+1.35em,
  row sep/small/.initial=+0.9em,
  row sep/tiny/.initial=+0.45em,
  column sep/huge/.initial=+4.8em,
  column sep/large/.initial=+3.6em,
  column sep/normal/.initial=+2.4em,
  column sep/scriptsize/.initial=+1.8em,
  column sep/small/.initial=+1.2em,
  column sep/tiny/.initial=+0.6em,
  crossing over clearance/.initial=+1.5ex,
  shift left/.default=+0.56ex,
  shift right/.default=1,
  background color/.initial=white}

% ConTeXt-specific stuff
\pgfutil@IfUndefined{starttikzpicture}{}{%
  \def\starttikzcd{\tikzcd}
  \def\stoptikzcd{\endtikzcd}
  \tikzcdset{
    every matrix/.append code={%
      \def\NC{\pgfmatrixnextcell}%
      \def\NR{\pgfmatrixendrow}}}
}

\endinput


==> mathdots/README <==
This is the mathdots package, version 0.9.
Copyright 2001--2014, Daniel H. Luecking

License:
=======
Mathdots may be distributed and/or modified under the conditions of the
LaTeX Project Public License, either version 1.3c of this license or (at
your option) any later version. The latest version of this license is in
   <http://www.latex-project.org/lppl.txt>
and version 1.3c or later is part of all distributions of LaTeX dated
2008/05/04 or later.

Mathdots has maintenance status "author-maintained". The Current
Maintainer is Daniel H. Luecking. The Base Interpreters associated with
mathdots are plain TeX and LaTeX

Purpose:
=======
This package changes the basic LaTeX and plain TeX commands \ddots and
\vdots so that they properly change size when font sizes change, and
when they are used in superscripts and subscripts. It also adds the
command \iddots (for inverse diagonal dots) which slants the opposite
way from \ddots.

In addition, if it detects amsmath in LaTeX (or AMSTeX in plain TeX) it
defines improved versions of the \dddot and \ddddot commands that place
three and four dots on a math symbol (similar to the math accent
commands \dot and \ddot). These also are arranged to change size
correctly and some placement bugs are corrected.

Other (minor) improvements: the commands \vdots, \ddots and \iddots
select the dot from the math fonts instead of the text fonts, so they
always match math punctuation dots. The \dddot and \ddddot commands
select the accent dot (same one placed by \dot).

File list:

README          This file
mathdots.dtx    The code
mathdots.pdf    The manual
mathdots.ins    unpacking script
mdotest.tex     LaTeX test file
plmdotest.tex   Plain TeX test file (requires loading amstex.tex and the
                and something to define the commands \eightpoint,
                \ninepoint, \tenpoint and \twelvepoint)

Installation:

Run tex or latex on mathdots.ins to unpack the files. Copy mathdots.tex
where tex will find it and mathdots.sty where latex will find it. Copy
the remaining files to your documentation area.

Daniel H. Luecking, \luecking \at \uark \dot \edu



==> mathdots/plmdotest.tex <==
\input amstex
\input mathdots

\eightpoint
eightpoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\ninepoint
ninepoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\tenpoint
tenpoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\twelvepoint
twelvepoint
$\ddots^{\ddots^{\ddots}}$ $\iddots^{\iddots^{\iddots}}$
$\vdots^{\vdots^{\vdots}}$

$\dot{X}$
$\ddot{X}$
$\dddot{X}$
$\ddddot{X}$
$X^{\dot{X}}$
$X^{\ddot{X}}$
$X^{\dddot{X}}$
$X^{\ddddot{X}}$
$X^{X^{\dot{X}}}$
$X^{X^{\ddot{X}}}$
$X^{X^{\dddot{X}}}$
$X^{X^{\ddddot{X}}}$

\smallskip
\hrule
\smallskip
\enddocument\end


==> mnsymbol/README <==
MnSymbol is a symbol font designed to be used in conjunction with Adobe
MinionPro.

All files in this archive are in the public domain.

WARNING
=======

This version includes a bugfix that causes incompatibilities with
previous versions. The symbols

  \...harpoonup and \...harpoondown

are now called

  \...harpoonccw and \...harpooncw

(This was needed for compatibility with amsfonts.sty.)

INSTALLATION
============

To install the fonts:

(0) If you have already a version of MnSymbol installed, delete the old
TFM and PK files.

(1) Run

  $ cd tex
  $ latex MnSymbol.ins

and copy the resulting file MnSymbol.sty to

   .../texmf/tex/latex/MnSymbol/MnSymbol.sty

(2) Copy all files in the "source" directory into the directory

   .../texmf/fonts/source/public/MnSymbol/

(3) Copy the documentation (MnSymbol.ps, MnSymbol.pdf, README) into the
directory

   .../texmf/doc/latex/MnSymbol/

(4) To install the PostScript fonts (courtesy of Michael Zedler) copy

  o enc/MnSymbol.map into .../texmf/fonts/map/dvips/MnSymbol
  o enc/*.enc        into .../texmf/fonts/enc/dvips/MnSymbol
  o pfb/*.pfb        into .../texmf/fonts/type1/public/MnSymbol

(These fonts are not strictly necessary but recommended.)

(5) You can copy the files in the "tfm" directory to

   .../texmf/fonts/tfm/public/MnSymbol

This is optional since these files can be generated automatically.
But it saves some time.

(6) Regenerate the file database:

  $ mktexlsr

If you installed the PostScript fonts you also need to run updmap or
updmap-sys to make them available:

  $ updmap-sys --enable MixedMap MnSymbol.map

(7) Happy TeXing.

Achim Blumensath


==> tikz-cd/tikzlibrarycd.code.tex <==
% tikzlibrarycd.code.tex [2018/11/19 v0.9f Commutative diagrams with TikZ]
%
% Copyright 2011, 2012, 2014, 2018 by Augusto Stoffel
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.

\usetikzlibrary{matrix,quotes,arrows.meta}

\newif\iftikzcd@mathmode

\def\tikzcdset{\pgfqkeys{/tikz/commutative diagrams}}

\tikzcdset{
  arrows/.code={\tikzcdset{every arrow/.append style={#1}}},
  labels/.code={\tikzcdset{every label/.append style={#1}}},
  cells/.code={\tikzcdset{every cell/.append style={#1}}},
  diagrams/.code={\tikzcdset{every diagram/.append style={#1}}},
  execute before arrows/.code={%
    \expandafter\def%
    \expandafter\tikzcd@before@paths@hook%
    \expandafter{\tikzcd@before@paths@hook#1}},
  to/.code={\tikzcd@setarrowend\tikzcd@ar@target{#1}},
  from/.code={\tikzcd@setarrowend\tikzcd@ar@start{#1}},
  shorten/.style={
    /tikz/shorten <=#1,
    /tikz/shorten >=#1},
  description/.style={
    /tikz/anchor=center,
    /tikz/fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color}},
  marking/.style={
    /tikz/font=,
    /tikz/sloped,
    /tikz/shape=asymmetrical rectangle,
    /tikz/anchor=center},
  phantom/.style={
    /tikz/draw=none,
    /tikz/commutative diagrams/labels={
      /tikz/font=,
      /tikz/anchor=center}},
  crossing over/.style={
    /tikz/preaction={
      /tikz/draw=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
      /tikz/arrows=-,
      /tikz/line width=\pgfkeysvalueof{/tikz/commutative diagrams/crossing over clearance}}},
  cramped/.code={\tikzcdset{
    every matrix/.append style={inner sep=+-0.3em},
    every cell/.append style={inner sep=+0.3em}}},
  row sep/.code={\tikzcd@sep{row}{#1}},
  column sep/.code={\tikzcd@sep{column}{#1}},
  sep/.code={\tikzcdset{row sep={#1},column sep={#1}}},
  math mode/.is if=tikzcd@mathmode,
  arrow style/.is choice}

\def\tikzcd@sep#1#2{%
  \pgfkeysifdefined{/tikz/commutative diagrams/#1 sep/#2}%
    {\pgfkeysgetvalue{/tikz/commutative diagrams/#1 sep/#2}\tikzcd@temp%
     \pgfkeysalso{/tikz/#1 sep/.expand once=\tikzcd@temp}}%
    {\pgfkeysalso{/tikz/#1 sep={#2}}}}

\def\tikzcd@setarrowend#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@\tikzcdmatrixname-#2}%
    {%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp#2\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef#1{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \def#1{#2}%
      \fi%
    }{%
      \def#1{\tikzcdmatrixname-#2}%
    }}
    
% The unknown key handler and direction argument parser
\tikzcdset{
  .unknown/.code={%
    \ifpgfkeysaddeddefaultpath%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp\pgfkeyscurrentname\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef\tikzcd@ar@target{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \pgfqkeys{/tikz}{\pgfkeyscurrentname={#1}}%
      \fi%
    \else%
      \def\pgfutilnext{\pgfkeysvalueof{/handlers/.unknown/.@cmd}#1\pgfeov}\pgfutilnext%
    \fi}}

\def\tikzcd@parse#1{% parser for arrow direction argument
  \ifx#1r\advance\c@pgf@countb by1\else%
   \ifx#1d\advance\c@pgf@counta by1\else%
    \ifx#1l\advance\c@pgf@countb by-1\else%
     \ifx#1u\advance\c@pgf@counta by-1\else%
      \ifx#1\relax\let\tikzcd@temp\pgfutil@empty%
       \else\let\tikzcd@temp\pgfutil@gobble@until@relax\fi\fi\fi\fi\fi%
  \tikzcd@temp}

% The `tikzcd' environment
\def\tikzcd{%
  \iffalse{\fi\ifnum0=`}\fi% standard trick to allow nesting of tabular-like environments (cf. the tabularx manual)
  \pgfutil@ifnextchar&% if we get an & here, it will be returned with the wrong catcode to the input stream
    {\expandafter\tikzcd@@\expandafter\pgfmatrixnextcell\pgfutil@gobble}%
    {\tikzcd@@}}

\def\tikzcd@@{\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@}{\tikzcd@[]}}

\def\tikzcd@[#1]{%
  \tikzpicture[/tikz/commutative diagrams/.cd,every diagram,#1]%
  \ifx\arrow\tikzcd@arrow%
    \pgfutil@packageerror{tikz-cd}{Diagrams cannot be nested}{}%
  \fi%
  \let\arrow\tikzcd@arrow%
  \let\ar\tikzcd@arrow%
  \def\rar{\tikzcd@xar{r}}%
  \def\lar{\tikzcd@xar{l}}%
  \def\dar{\tikzcd@xar{d}}%
  \def\uar{\tikzcd@xar{u}}%
  \def\urar{\tikzcd@xar{ur}}%
  \def\ular{\tikzcd@xar{ul}}%
  \def\drar{\tikzcd@xar{dr}}%
  \def\dlar{\tikzcd@xar{dl}}%
  \global\let\tikzcd@savedpaths\pgfutil@empty%
  \matrix[%
    /tikz/matrix of \iftikzcd@mathmode math \fi nodes,%
    /tikz/every cell/.append code={\tikzcdset{every cell}},%
    /tikz/commutative diagrams/.cd,every matrix]%
  \bgroup}

\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths%
  \endgroup%
  \endtikzpicture%
  \ifnum0=`{}\fi}

% The arrow commands
\def\tikzcd@arrow{%
  \relax% this was added to avoid errors when a cell starts with \arrow, but it seems unnecessary now
  \edef\tikzcd@temp{%
    \noexpand\def\noexpand\tikzcd@currentcolumn{\the\pgfmatrixcurrentcolumn}%
    \noexpand\def\noexpand\tikzcd@currentrow{\the\pgfmatrixcurrentrow}%
    \noexpand\def\noexpand\tikzcd@lineno{\the\inputlineno}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@savedpaths\expandafter{\tikzcd@temp}%
  \pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@arrow}{\tikzcd@ar@old[]}}

\def\tikzcd@@arrow[#1]{\pgfutil@ifnextchar\bgroup{\tikzcd@ar@old[#1]}{\tikzcd@ar@new[#1]}}

\def\tikzcd@ar@new[#1]{% new syntax
  \pgfutil@g@addto@macro\tikzcd@savedpaths{%
    \path[/tikz/commutative diagrams/.cd,every arrow,#1]%
    (\tikzcd@ar@start\tikzcd@startanchor) to (\tikzcd@ar@target\tikzcd@endanchor); }}

\def\tikzcd@ar@old[#1]#2{% old syntax
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{to={#2},#1}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{to={#2},#1}[]}%
      {\tikzcd@ar@new[to={#2},#1]}}}

\def\tikzcd@ar@getlabel#1[#2]#3{%
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{#1,"{#3}"{#2}}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{#1,"{#3}"{#2}}[]}%
      {\tikzcd@ar@new[#1,"{#3}"{#2}]}}}

\def\tikzcd@xar#1{\relax\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@xar{#1}}{\tikzcd@arrow[]{#1}}}
\def\tikzcd@@xar#1[#2]{\tikzcd@arrow[#2]{#1}}

\def\tikzcd@handle@shortcuts@next{% expand next macro using standard catcodes
  \iftikz@handle@active@code%
    \begingroup%
      \tikz@switchoff@shorthands\expandafter%
    \endgroup\expandafter%
  \fi}

\def\tikzcd@ar@target{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}
\def\tikzcd@ar@start{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}

\def\tikzcd@forward@quotes#1{\tikzset{every to/.append style={#1}}}

\let\tikzcd@before@paths@hook\pgfutil@empty

% `start anchor', `end anchor', and `shift' keys
\def\tikzcd@setanchor#1[#2]#3\relax{%
  \ifx\relax#2\relax\else%
    \tikzcdset{@#1transform/.append style={#2},@shiftabletopath}%
  \fi%
  \ifx\relax#3\relax%
    \pgfutil@namelet{tikzcd@#1anchor}{pgfutil@empty}%
  \else%
    \pgfutil@namedef{tikzcd@#1anchor}{.#3}%
  \fi}

\tikzcdset{
  @shiftabletopath/.style={
    /tikz/execute at begin to={%
      \begingroup%
        \def\tikz@tonodes{coordinate[pos=0,commutative diagrams/@starttransform/.try](tikzcd@nodea) %
                          coordinate[pos=1,commutative diagrams/@endtransform/.try](tikzcd@nodeb)}%
        \path (\tikztostart) \tikz@to@path;%
      \endgroup%
      \def\tikztostart{tikzcd@nodea}%
      \def\tikztotarget{tikzcd@nodeb}%
      \tikzset{insert path={(tikzcd@nodea)}}},
    /tikz/commutative diagrams/@shiftabletopath/.code={}},
  start anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{start}}{\tikzcd@setanchor{start}[]}#1\relax},%]
  end anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{end}}{\tikzcd@setanchor{end}[]}#1\relax},%]
  start anchor=,
  end anchor=,
  shift left/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/execute at begin to={%
      \pgfpointnormalised{%
        \pgfpointdiff{\pgfpointanchor{tikzcd@nodeb}{center}}{\pgfpointanchor{tikzcd@nodea}{center}}}%
      \pgfgetlastxy{\tikzcd@x}{\tikzcd@y}%
      \pgfmathparse{#1}%
      \ifpgfmathunitsdeclared\else
        \pgfmathparse{\pgfmathresult*\pgfkeysvalueof{/tikz/commutative diagrams/shift left/.@def}}
      \fi
      \coordinate (tikzcd@nodea) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodea);%
      \coordinate (tikzcd@nodeb) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodeb);%
      \tikzset{insert path={(tikzcd@nodea)}}}},
  shift right/.style={
    /tikz/commutative diagrams/shift left={-(#1)}},
  transform nodes/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/commutative diagrams/@starttransform/.append style={#1},
    /tikz/commutative diagrams/@endtransform/.append style={#1}},
  shift/.style={
    /tikz/shift={#1},% we need this for labels to receive a shift
    /tikz/commutative diagrams/transform nodes={/tikz/shift={#1}}},
  xshift/.style={
    /tikz/xshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/xshift={#1}}},
  yshift/.style={
    /tikz/yshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/yshift={#1}}}}

% pgfmath functions to obtain math fontdimens
\pgfutil@ifluatex

  \directlua{tex.enableprimitives('tikzcd@', {'Umathaxis', 'Umathfractionrule'})}

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\tikzcd@Umathaxis\textstyle%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\tikzcd@Umathfractionrule\textstyle%
    \endgroup}

\else% if using (pdf)tex

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\fontdimen22\textfont2%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\fontdimen8\textfont3%
    \endgroup}

\fi

% The shape used inside matrices
\pgfdeclareshape{asymmetrical rectangle} {
  \inheritsavedanchors[from={rectangle}]
  \inheritanchor[from={rectangle}]{base}
  \inheritanchor[from={rectangle}]{north}
  \inheritanchor[from={rectangle}]{south}
  \inheritanchor[from={rectangle}]{base west}
  \inheritanchor[from={rectangle}]{north west}
  \inheritanchor[from={rectangle}]{south west}
  \inheritanchor[from={rectangle}]{base east}
  \inheritanchor[from={rectangle}]{north east}
  \inheritanchor[from={rectangle}]{south east}
  \inheritanchor[from={rectangle}]{mid}
  \inheritanchor[from={rectangle}]{mid west}
  \inheritanchor[from={rectangle}]{mid east}
  \inheritbackgroundpath[from={rectangle}]
  \anchor{center}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{west}{\pgf@anchor@rectangle@west\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{east}{\pgf@anchor@rectangle@east\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{real center}{\pgf@anchor@rectangle@center}
  \anchor{real west}{\pgf@anchor@rectangle@west}
  \anchor{real east}{\pgf@anchor@rectangle@east}
  \anchorborder{%
    \pgfmathsetlength\pgfutil@tempdima%
      {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \ifdim\pgf@yb>0pt%
      \northeast%
      \pgf@yc=\pgf@y%
      \advance\pgf@yc by-\pgfutil@tempdima%
    \else%
      \southwest%
      \pgf@yc=-\pgf@y%
      \advance\pgf@yc by\pgfutil@tempdima%
    \fi
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgfutil@tempdima%
  }%
}%

% Computer modern arrow tips
\pgfkeys{
  cm to/.tip={Computer Modern Rightarrow[length=+0pt 6.2]},
  cm bold to/.tip={cm to[scale=0.667]},
  cm double to/.tip={cm to[sep=+0pt -2.6]cm to},
  cm bar/.tip={Bar[width=+0pt 8.2 0.89,line cap=round]},
  cm left hook/.tip={Hooks[width=+0pt 10.8,length=+0pt 3.6,harpoon,line cap=round]},
  cm implies/.tip={Implies},
  cm left to/.tip={cm to[left]},
  cm right to/.tip={cm to[right]},
  cm right hook/.tip={cm left hook[swap]},
  cm to reversed/.tip={cm to[reversed]},
  cm */.tip={Circle[length=+0pt 7.6]},
  cm o/.tip={cm *[open]},
  cm |/.tip={cm bar}}%|

% The `Glyph' meta arrow tip
\pgfqkeys{/pgf/arrow keys}{
  glyph math command/.code={% if csname #1 is undefined, we want it to remain so
    \pgfarrowsaddtooptions{\def\tikzcd@glyph{$\begingroup\expandafter\endgroup\csname #1\endcsname$}}},
  glyph axis/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@axis{#1}}},
  glyph length/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@len{#1}}},
  glyph shorten/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@shorten{#1}}}}

\pgfdeclarearrow{
  name=Glyph,
  cache=false,
  bending mode=none,
  parameters={\tikzcd@glyph@len,\tikzcd@glyph@shorten},
  setup code={%
    \pgfarrowssettipend{\tikzcd@glyph@len\advance\pgf@x by\tikzcd@glyph@shorten}},
  defaults={
    glyph axis=axis_height,
    glyph length=+0.9ex,
    glyph shorten=+-0.1ex},
  drawing code={%
    \pgfpathrectangle{\pgfpoint{+0pt}{+-1ex}}{\pgfpoint{+\tikzcd@glyph@len}{+2ex}}%
    \pgfusepathqclip%
    \pgftransformxshift{+\tikzcd@glyph@len}%
    \pgftransformyshift{+-\tikzcd@glyph@axis}%
    \pgftext[right,base]{\tikzcd@glyph}}}

% Arrow tip selection styles
\tikzcdset{
  double line/.code={\tikzset{%
    double equal sign distance,
    double=\pgfkeysvalueof{/tikz/commutative diagrams/background color}}},
  dashed/.style={/tikz/dash pattern={on 7\pgflinewidth off 4\pgflinewidth}},
  tikzcd to/.tip={cm to},
  tikzcd bar/.tip={cm bar},
  tikzcd left hook/.tip={cm left hook},
  tikzcd double to/.tip={cm double to},
  tikzcd implies/.tip={Implies},
  tikzcd right hook/.tip={tikzcd left hook[swap]},
  tikzcd left to/.tip={tikzcd to[harpoon]},
  tikzcd right to/.tip={tikzcd left to[swap]},
  tikzcd to reversed/.tip={tikzcd to[reversed]},
  tikzcd cap/.tip={},
  tikzcd implies cap/.tip={},
  tikzcd implies bar/.tip={tikzcd bar},
  no tail/.code={\pgfsetarrowsstart{tikzcd cap}},
  to head/.code={\pgfsetarrowsend{tikzcd to}},
  maps to/.code={\pgfsetarrowsstart{tikzcd bar}},
  hook/.code={\pgfsetarrowsstart{tikzcd right hook}},
  hook'/.code={\pgfsetarrowsstart{tikzcd left hook}},
  harpoon/.code={\pgfsetarrowsend{tikzcd left to}},
  harpoon'/.code={\pgfsetarrowsend{tikzcd right to}},
  two heads/.code={\pgfsetarrowsend{tikzcd double to}},
  tail/.code={\pgfsetarrowsstart{tikzcd to reversed}},
  rightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd to}},
  Rightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies}},
  leftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd cap}},
  Leftarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies cap}},
  leftrightarrow/.code={\pgfsetarrows{tikzcd to-tikzcd to}},
  Leftrightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies}},
  mapsto/.code={\pgfsetarrows{tikzcd bar-tikzcd to}},
  mapsfrom/.code={\pgfsetarrows{tikzcd to-tikzcd bar}},
  Mapsto/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies bar-tikzcd implies}},
  Mapsfrom/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies bar}},
  hookrightarrow/.code={\pgfsetarrows{tikzcd right hook-tikzcd to}},
  hookleftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd left hook}},
  rightharpoonup/.code={\pgfsetarrows{tikzcd cap-tikzcd left to}},
  rightharpoondown/.code={\pgfsetarrows{tikzcd cap-tikzcd right to}},
  leftharpoonup/.code={\pgfsetarrows{tikzcd right to-tikzcd cap}},
  leftharpoondown/.code={\pgfsetarrows{tikzcd left to-tikzcd cap}},
  rightarrowtail/.code={\pgfsetarrows{tikzcd to reversed-tikzcd to}},
  leftarrowtail/.code={\pgfsetarrows{tikzcd to-tikzcd to reversed}},
  twoheadrightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd double to}},
  twoheadleftarrow/.code={\pgfsetarrows{tikzcd double to-tikzcd cap}},
  no head/.code={\pgfsetarrowsend{tikzcd cap}},
  dash/.code={\pgfsetarrows{tikzcd cap-tikzcd cap}},
  dashrightarrow/.code={\tikzcdset{rightarrow,dashed}},
  dashleftarrow/.code={\tikzcdset{leftarrow,dashed}},
  equal/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies cap}},
  equals/.code={\tikzcdset{equal}},
  rightsquigarrow/.code={\tikzcdset{rightarrow,squiggly}},
  leftsquigarrow/.code={\tikzcdset{leftarrow,squiggly}},
  leftrightsquigarrow/.code={\tikzcdset{leftrightarrow,squiggly}},
  squiggly/.code={%
    \pgfutil@ifundefined{tikz@library@decorations.pathmorphing@loaded}%
      {\pgfutil@packageerror{tikz-cd}{You need to say %
      \string\usetikzlibrary{decorations.pathmorphing} to use squiggly arrows}{}}{}%
    \pgfkeysalso{
      /tikz/decorate,
      /tikz/decoration={
        zigzag,
        segment length=9.25\pgflinewidth,
        amplitude=1.9\pgflinewidth,
        post=lineto, post length=6\pgflinewidth,
        pre=lineto, pre length=6\pgflinewidth,
        #1}}}}

% The `Latin Modern' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/Latin Modern}{%
  \tikzcdset{
    tikzcd bar/.tip={Bar[width=+0pt 12 .992,line cap=round]},
    tikzcd left hook/.tip={Hooks[width=+0pt 15,length=+0pt 4.2,arc=190,harpoon,line cap=round]}}}

% The `tikz' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/tikz}{%
  \tikzcdset{
    tikzcd to/.tip={>},
    tikzcd bar/.tip={Bar[width=+3pt 4 0.9]},
    tikzcd left hook/.tip={Hooks[harpoon]},
    tikzcd double to/.tip={tikzcd to[]tikzcd to}}}

% The `math font' arrow style
%
% If your font does not define the command \mapsfrom, do so by saying
%   \def\mapsfrom{\pgfpicture\pgfsetbaseline{+0pt}\pgftransformxscale{-1}\pgftext[base]{$\mapsto$}\endpgfpicture}
%
% The method used to guess the correct value of `double distance'
% inside the `double line' style is not robust at all.  If it fails,
% set
%   \tikzcdset{double line/.append style={double distance=2*rule_thickness}}
% and find the correct value for `double distance' by trial and error
% (or measure the distance between the \Rightarrow stems in a font
% editor).
%
\pgfkeysdef{/tikz/commutative diagrams/arrow style/math font}{%
  \tikzcdset{
    tikzcd to/.tip={Glyph[glyph math command=rightarrow]},
    tikzcd cap/.tip={Glyph[glyph math command=leftarrow]},
    tikzcd to reversed/.tip={Glyph[glyph math command=leftarrowtail]},
    tikzcd bar/.tip={Glyph[glyph math command=mapsfrom]},
    tikzcd left hook/.tip={Glyph[glyph math command=hookleftarrow]},
    tikzcd right hook/.tip={Glyph[glyph math command=hookleftarrow, swap]},
    tikzcd implies/.tip={Glyph[glyph math command=Rightarrow, glyph length=1.2ex]},
    tikzcd implies cap/.tip={Glyph[glyph math command=Leftarrow]},
    tikzcd implies bar/.tip={Glyph[glyph math command=Mapsfrom]},
    tikzcd double to/.tip={Glyph[glyph math command=twoheadrightarrow, glyph length=1.4ex]},
    tikzcd left to/.tip={Glyph[glyph math command=rightharpoonup]},
    tikzcd right to/.tip={Glyph[glyph math command=rightharpoonup,swap]},
    double line/.append code={\tikzset{double distance={2*(height("$=$")-axis_height-rule_thickness)}}},
    dashed/.code={\tikzset{dash pattern=on 0.8ex off 0.4ex, dash phase=0.8ex}},
    squiggly/.default={pre length=1ex, post length=1ex}}}

% Default settings
\tikzcdset{
  every arrow/.style={
    /tikz/draw,
    /tikz/line width=rule_thickness,
    /tikz/commutative diagrams/rightarrow},
  every label/.style={
    /tikz/auto,
    /tikz/font=\everymath\expandafter{\the\everymath\scriptstyle},
    /tikz/inner sep=+0.5ex},
  every cell/.style={
    /tikz/shape={asymmetrical rectangle},
    /tikz/inner xsep=+1ex,
    /tikz/inner ysep=+0.85ex},
  every matrix/.style={/tikz/inner sep=+0pt},
  every diagram/.style={
    /tikz/commutative diagrams/row sep=normal,
    /tikz/commutative diagrams/column sep=normal,
    /tikz/baseline=+0pt},
  1-row diagram/.style={/tikz/baseline/.expanded=(\tikzcdmatrixname.base)},
  math mode=true,
  center yshift/.initial=axis_height,
  row sep/huge/.initial=+3.6em,
  row sep/large/.initial=+2.7em,
  row sep/normal/.initial=+1.8em,
  row sep/scriptsize/.initial=+1.35em,
  row sep/small/.initial=+0.9em,
  row sep/tiny/.initial=+0.45em,
  column sep/huge/.initial=+4.8em,
  column sep/large/.initial=+3.6em,
  column sep/normal/.initial=+2.4em,
  column sep/scriptsize/.initial=+1.8em,
  column sep/small/.initial=+1.2em,
  column sep/tiny/.initial=+0.6em,
  crossing over clearance/.initial=+1.5ex,
  shift left/.default=+0.56ex,
  shift right/.default=1,
  background color/.initial=white}

% ConTeXt-specific stuff
\pgfutil@IfUndefined{starttikzpicture}{}{%
  \def\starttikzcd{\tikzcd}
  \def\stoptikzcd{\endtikzcd}
  \tikzcdset{
    every matrix/.append code={%
      \def\NC{\pgfmatrixnextcell}%
      \def\NR{\pgfmatrixendrow}}}
}

\endinput

